Deep Portrait Quality Assessment. A NTIRE 2024 Challenge Survey

This paper reviews the NTIRE 2024 Portrait Quality Assessment Challenge, highlighting the proposed solutions and results. This challenge aims to obtain an efficient deep neural network capable of estimating the perceptual quality of real portrait photos. The methods must generalize to diverse scenes and diverse lighting conditions (indoor, outdoor, low-light), movement, blur, and other challenging conditions. In the challenge, 140 participants registered, and 35 submitted results during the challenge period. The performance of the top 5 submissions is reviewed and provided here as a gauge for the current state-of-the-art in Portrait Quality Assessment.

==> teams/team6.tex <==
\subsection{Portrait Quality Assessment by Self-Adaptive Hyper Network}

%%%%%%%%%%% PLEASE FILL THIS INFORMATION WITH YOUR TEAM'S DETAILS
%%%% IF THE INFORMATION DOES NO MATCH THE FACTSHEET, WE WILL NOT INCLUDE IT

\begin{center}

\vspace{2mm}
\noindent\emph{\textbf{Team Panmoon}}
\vspace{2mm}

\noindent\emph{Yueliang Pan, Qisheng Xu, Kele Xu, Long Lan}

\vspace{2mm}

\noindent\emph{
National University of Defense Technology}


\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/team6.png}
    \caption{The pipeline of the HyperIQA network.}
    \label{fig:team_6}
\end{figure*}

This method dissects the Portrait Quality Assessment (PQA) procedure into three distinct stages: content understanding, perception rule learning, and quality prediction. Following the extraction of image semantics, the perception rule is dynamically established by a hyper-network and subsequently utilized by a quality prediction network.

We opted to fine-tune the HyperIQA~\cite{9156687} model using the officially released PIQ23 dataset, known for its strong validation across the majority of IQA datasets. This model possesses the capability to adaptively predict image quality based on the content of the images. Given the diverse range of image types typically present in IQA evaluation datasets, we trained the HyperIQA model on the overall part of the PIQ23 dataset according to partition requirements, aiming to further specialize it in the domain of human portrait quality assessment.

During training, we adhered to the training strategy utilized by the original model when trained on the LIVEC dataset. Subsequently, new parameters were obtained after training for approximately 100 epochs on the PIQ23 dataset. During inference, these new parameters were employed to infer each image once.



The model network comprises three main components, as illustrated in Figure \ref{fig:team_6}: a backbone network responsible for extracting semantic features $S(x)$, a target network designed to predict image quality score $q$, and a hyper network tasked with learning the quality perception rule $\theta_x$  to generate a series of self-adaptive parameters for the target network. Specifically, we employed ResNet50 as the backbone model for semantic feature extraction, initializing it with a pre-trained model on ImageNet. The target network, consisting of four fully connected layers, receives a multi-scale content feature vector as input and undergoes propagation through weight-determined layers to yield the final quality score. Within the target network, we employed the sigmoid function as the activation function. The hyper network comprises three $1\times1$ convolution layers and several weight-generating branches.
\\


\paragraph{Implementation details}

We implemented our model by PyTorch and conducted training and testing on a NVIDIA 3090 GPU. Following the original model training strategy on the LIVEC dataset, we randomly sample and horizontally flipping 25 patches with size $224\times 224$ pixels from each training image for augmentation. Training patches inherited quality scores from the source image, and we minimize $L_1$ loss over the training set:
 
\begin{equation}
     l = \frac{1}{N}\sum\limits_{N}^{t}\Vert \varphi(v_{p_i}, H(S(p_i), \gamma))-Q_i \Vert_2
\end{equation}
where $p_i$ and $Q_i$ refers to the $i$-th training patch and the ground truth score, respectively. We used Adam optimizer with weight decay $5 \times 10^{-4}$ to train our model for 100 epochs, with mini-batch size of 8. Learning rate is first set to $2 \times 10^{-5}$, and reduced by 10 after every 5 epochs. For faster convergence, un-pretrained layers of our model, which are Xavier initialized, applied learning rate 10 times larger. We save the parameters obtained after each training iteration and select the parameters from the iteration with the lowest training loss as the new parameters.During the inference process, we found that employing our new parameters results in the same output for each image after averaging the results of ten inference runs using the original strategy, as compared to a single run. Therefore, only one inference run is necessary during the inference process.
